Understanding Communication Preferences of Information Workers in Engagement with Text-Based Conversational Agents

Communication traits in text-based human-AI conversations play pivotal roles in shaping user experiences and perceptions of systems. With the advancement of large language models (LLMs), it is now feasible to analyze these traits at a more granular level. In this study, we explore the preferences of information workers regarding chatbot communication traits across seven applications. Participants were invited to participate in an interactive survey, which featured adjustable sliders, allowing them to adjust and express their preferences for five key communication traits: formality, personification, empathy, sociability, and humor. Our findings reveal distinct communication preferences across different applications; for instance, there was a preference for relatively high empathy in wellbeing contexts and relatively low personification in coding. Similarities in preferences were also noted between applications such as chatbots for customer service and scheduling. These insights offer crucial design guidelines for future chatbots, emphasizing the need for nuanced trait adjustments for each application.

==> Draft/findings.tex <==
\section{Findings}


% Table \ref{ref: avg_pref} shows the average preferences participants provided for all communication traits for different applications. Figure \ref{fig:avg_scores} groups these average scores side-by-side for easy visualization. 

% \input{Tables-Figures/avg-preference}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9\linewidth]{Tables-Figures/Avg_User_Preference_Scores.png}
%     \caption{Average User Preference Scores for Communication Traits Across Applications}
%     \label{fig:avg_scores}
% \end{figure}

\subsection{Formality}
%\subsection{Formality}
\begin{figure}[h!]
    \centering
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Formality_Scores.png}
        \caption{Average User Preference Scores for Formality Across All Applications}
        \label{fig:formality_scores}
    \end{minipage}\hfill
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Histogram_Formality.png}
        \caption{Histograms of User Preference Scores for Formality Across All Applications}
        \label{fig:histogram_formality}
    \end{minipage}
\end{figure}


\todo{explanation}

\todo{Formality Distribution}


\todo{Statistics}
\input{Tables-Figures/formality-table}



\subsection{Validation}

\todo{check}


==> Tables-Figures/avg-preference.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\textbf{Application} & \textbf{Formality} & \textbf{Personification} & \textbf{Empathy} & \textbf{Sociability} & \textbf{Humor} \\ \hline
Customer Service  & 2.89 $\pm$ 0.07 & 2.62 $\pm$ 0.07 & 2.97 $\pm$ 0.08 & 2.45 $\pm$ 0.07 & 1.78 $\pm$ 0.06 \\ \hline
Coding            & 2.80 $\pm$ 0.08 & 2.13 $\pm$ 0.06 & 2.14 $\pm$ 0.07 & 1.99 $\pm$ 0.06 & 1.82 $\pm$ 0.06 \\ \hline
Time Management   & 2.64 $\pm$ 0.07 & 2.71 $\pm$ 0.07 & 2.69 $\pm$ 0.07 & 2.44 $\pm$ 0.06 & 2.09 $\pm$ 0.06 \\ \hline
Wellbeing         & 2.39 $\pm$ 0.06 & 2.92 $\pm$ 0.07 & 3.41 $\pm$ 0.07 & 2.90 $\pm$ 0.07 & 2.13 $\pm$ 0.06 \\ \hline
Gaming            & 2.09 $\pm$ 0.06 & 2.80 $\pm$ 0.07 & 2.50 $\pm$ 0.07 & 2.64 $\pm$ 0.06 & 2.57 $\pm$ 0.07 \\ \hline
Story Writing     & 2.49 $\pm$ 0.07 & 3.07 $\pm$ 0.07 & 2.84 $\pm$ 0.07 & 2.92 $\pm$ 0.07 & 2.67 $\pm$ 0.07 \\ \hline
Information Retrieval & 2.75 $\pm$ 0.07 & 2.49 $\pm$ 0.07 & 2.35 $\pm$ 0.07 & 2.38 $\pm$ 0.06 & 1.96 $\pm$ 0.06 \\ \hline
All Scenarios     & 2.58 $\pm$ 0.18 & 2.68 $\pm$ 0.18 & 2.70 $\pm$ 0.19 & 2.53 $\pm$ 0.18 & 2.14 $\pm$ 0.17 \\ \hline
\end{tabular}
\caption{Scores for different traits across various scenarios}
\label{ref: avg_pref}
\end{table}


==> Tables-Figures/corr_traits.tex <==
\begin{table}[H]
\centering
\caption{Average Correlation Matrix for All Communication Traits}
\label{tab:correlation_matrix_traits}
\begin{tabular}{|c|c|c|c|c|c|}\hline
{} & \textbf{Formality} & \textbf{Personification} & \textbf{Empathy} & \textbf{Sociability} & \textbf{Humor} \\\hline
\textbf{Formality}    & 1.00 & 0.03 & 0.02 & -0.02 & -0.11 \\\hline
\textbf{Personification} & 0.03 & 1.00 & 0.43 & 0.53 & 0.32 \\\hline
\textbf{Empathy}       & 0.02 & 0.43 & 1.00 & 0.51 & 0.37 \\\hline
\textbf{Sociability}   & -0.02 & 0.53 & 0.51 & 1.00 & 0.40 \\\hline
\textbf{Humor}         & -0.11 & 0.32 & 0.37 & 0.40 & 1.00 \\\hline
\end{tabular}
\end{table}


==> Tables-Figures/formality-table.tex <==
\begin{table}[h!]
\centering
\caption{Significance Matrix for Formality}
\label{tab:sig_matrix}
\begin{tabular}{l*{7}{c}}
\hline
 & \textbf{Customer} & \textbf{Coding} & \textbf{Scheduling} & \textbf{Wellbeing} & \textbf{Gaming} & \textbf{Story} & \textbf{Info} \\ 
\hline
\textbf{Customer} & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} \\
\hline
\textbf{Coding} & \cellcolor{falsecolor}False & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} \\
\hline
\textbf{Scheduling} & \cellcolor{truecolor}True & \cellcolor{falsecolor}False & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} \\
\hline
\textbf{Wellbeing} & \cellcolor{truecolor}True & \cellcolor{truecolor}True & \cellcolor{truecolor}True & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} \\
\hline
\textbf{Gaming} & \cellcolor{truecolor}True & \cellcolor{truecolor}True & \cellcolor{truecolor}True & \cellcolor{truecolor}True & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} \\
\hline
\textbf{Story} & \cellcolor{truecolor}True & \cellcolor{truecolor}True & \cellcolor{falsecolor}False & \cellcolor{falsecolor}False & \cellcolor{truecolor}True & \cellcolor{white} & \cellcolor{white} \\
\hline
\textbf{Info} & \cellcolor{falsecolor}False & \cellcolor{falsecolor}False & \cellcolor{falsecolor}False & \cellcolor{truecolor}True & \cellcolor{truecolor}True & \cellcolor{truecolor}True & \cellcolor{white} \\
\hline
\end{tabular}
\end{table}
